Interactive Debugging of Knowledge Bases

Many AI applications rely on knowledge about a relevant real-world domain that is encoded by means of some logical knowledge base (KB). The most essential benefit of logical KBs is the opportunity to perform automatic reasoning to derive implicit knowledge or to answer complex queries about the modeled domain. The feasibility of meaningful reasoning requires KBs to meet some minimal quality criteria such as logical consistency. Without adequate tool assistance, the task of resolving violated quality criteria in KBs can be extremely tough even for domain experts, especially when the problematic KB includes a large number of logical formulas or comprises complicated logical formalisms. Published non-interactive debugging systems often cannot localize all possible faults (incompleteness), suggest the deletion or modification of unnecessarily large parts of the KB (non-minimality), return incorrect solutions which lead to a repaired KB not satisfying the imposed quality requirements (unsoundness) or suffer from poor scalability due to the inherent complexity of the KB debugging problem. Even if a system is complete and sound and considers only minimal solutions, there are generally exponentially many solution candidates to select one from. However, any two repaired KBs obtained from these candidates differ in their semantics in terms of entailments and non-entailments. Selection of just any of these repaired KBs might result in unexpected entailments, the loss of desired entailments or unwanted changes to the KB. This work proposes complete, sound and optimal methods for the interactive debugging of KBs that suggest the one (minimally invasive) error correction of the faulty KB that yields a repaired KB with exactly the intended semantics. Users, e.g. domain experts, are involved in the debugging process by answering automatically generated queries about the intended domain.

==> conclusion.tex <==
\chapter{Future Work}
\label{chap:conclusion}
%\fixme{include short discussion on hierarchical reasoning and mention MORe by Horrocks}
%CONCLUSION + SUMMARY

%\noindent\textbf{Summary.}


\subsubsection*{Topics for Future Work}
	\label{sec:future_work}
This work has given rise to several questions we will elaborate on in our future work: 

\noindent\textbf{Query Generation and Selection.}
%\begin{itemize}
	%\item Of course, these assumptions and methods of obtaining fault probabilities of syntactical elements and formulas are only \emph{some} possible ways of doing so. For example, one might argue that the ``authorship'' of a formula is somewhat not clearly defined. What if user $u_1$ has originally written formula $\tax$ and then user $u_2$ alters the formula to become $\tax'$? Who is the author of $\tax'$? $u_1$, $u_2$ or both? For whose fault probability computation should the renewed modification of $\tax'$ to $\tax''$ count? Questions like this one need to be discussed and maybe evaluations using real data need to be accomplished in order to find a practical answer; or perhaps to find out that completely different approaches turn out to be reasonable. This is a topic of our future work.
	%\item 
Our discussions of the presented query generation methods have revealed some drawbacks (cf.\ Chapter~\ref{chap:QueryGeneration}). Albeit being a fixed-parameter tractable problem as argued, the exponential time complexity regarding the number of leading diagnoses $|\mD|$ in case an optimal query 
	%with optimal information theoretic properties such as information gain 
	is desired is clearly an aspect that should be improved. This high complexity arises from the paradigm of computing an optimal query w.r.t.\ some measure $qsm()$ by calculating a (generally exponentially large) pool $\QP$ of queries in a first stage, whereupon the best query in $\QP$ according to $qsm()$ is filtered out in a second stage.
	
	A key to solving this issue is the use of a different paradigm that does not rely on the computation of the pool $\QP$. Instead, qualitative measures can be derived from quantitative measures that have been used in interactive debugging scenarios~\cite{Shchekotykhin2012, Rodler2013, ksgf2010}. These qualitative measures provide a way to estimate the $qsm()$ value of \emph{partial q-partitions}, i.e.\ ones where not all leading diagnoses have been assigned to the respective set in the q-partition yet. In this way a \emph{direct} search for a query with (nearly) optimal properties is possible. A similar strategy called CKK has been employed in~\cite{Shchekotykhin2012} for the information gain measure $qsm() := \mathsf{ENT()}$ (see Section~\ref{sec:query_selection_measures}). From such a technique we can expect to save a high number of reasoner calls. Because usually only a small subset of q-partitions included in a query pool (of exponential cardinality) is required to find a query with desirable properties if the search is implemented by means of a \emph{heuristic} that involves the exploration of seemingly favorable (potential) queries and (partial) q-partitions, respectively, first. 

Another shortcoming of the paradigm of query pool generation and subsequent selection of the best query is the extensive use of reasoning services which may be computationally expensive (depending on the given DPI). Instead of computing a set of common entailments $Q$ of a set of KBs $\mo_i^*$ first and consulting a reasoner to fill up the (q-)partition for $Q$ in order to test whether $Q$ is a query at all (see Chapter~\ref{chap:QueryGeneration}), the idea enabling a significant reduction of reasoner dependence is to compute some kind of \emph{canonical query} without a reasoner and use simple set comparisons to decide whether the associated partition is a q-partition. Guided by qualitative properties mentioned before, a search for such q-partition with desirable properties can be accomplished \emph{without reasoning at all}. Also, a set-minimal version of the optimal canonical query can be computed without reasoning aid. Only for the optional enrichment of the identified optimal canonical query by additional entailments and for the subsequent minimization of the enriched query, the reasoner may be employed. We will present strategies accounting for these ideas in the near future.

Another aspect that can be improved is that \emph{only one} minimized version of each query is computed by Algorithm~\ref{algo:query_gen}. That is, per q-partition $\Pt$, there might be some set-minimal queries which do not occur in the output set $\QP$. From the point of view of how well a query might be understood by an interacting user, of course not all minimized queries can be assumed equally good in general. For instance, consider the minimized queries $Q_4$ and $Q_{10}$ in Table~\ref{tab:queries_partitions} on page~\pageref{tab:queries_partitions}. Both are equally good regarding their q-partitions (just the sets $\dx{}$ and $\dnx{}$ are commuted), but most people will probably agree that $Q_4$ is much easier to comprehend from the logical point of view and thus much easier to answer.

Hence, in order to avoid a situation where a potentially best-understood query w.r.t.\ $\Pt$ is not included in $\QP$, the query minimization process (see Section~\ref{sec:minimization_of_queries}) might be adapted to take into account some information about faults the interacting user is prone to. This could be exploited to estimate how well this user might be able to understand and answer a query. For instance, given that the user frequently has problems to apply $\exists$ in a correct manner to express what they intend to express, but has never made any mistakes in formulating implications $\rightarrow$, then the query $Q_1 = \setof{\forall X\,p(X) \rightarrow q(X), r(a)}$ might be better comprehended than $Q_2 = \setof{\forall X \exists Y s(X,Y)}$. One way to achieve the finding of a well-understood query for some q-partition $\Pt$ is to run the query minimization \textsc{minQ} more than once, each time with a modified input (using a hitting set tree to accomplish this in a systematic manner -- cf.\ Chapter~\ref{chap:DiagnosisComputation}, where an analogue idea is used to compute different minimal conflict sets w.r.t.\ a DPI). In this way, different set-minimal queries for $\Pt$ can be identified and the process can be stopped when a suitable query is found. 

In order to come up with such a strategy, however, one must first gain insight into how well a user might understand certain logical formalisms and what properties make a query easy to comprehend from the logical perspective. It is planned to gather corresponding data about different users in the scope of a user study and to utilize the results to achieve a model of ``query hardness'' (by sticking to a similar overall methodology as used in \cite{Horridge2011b}) in order to come up with strategies for the determination of minimal queries that are easily understood. Note that such a model could also act as a guide how to specify the initial fault probabilities of syntactical elements that are used to obtain diagnoses probabilities (see Section~\ref{sec:DiagnosisProbabilitySpace}).

\noindent\textbf{Incorporating A-Posteriori Probabilities into Diagnosis Search.} As we discussed in Remark~\ref{rem:absolute_vs_relative_fault_tolerance_AND_initial_vs_updated_probabilities} on page~\pageref{rem:absolute_vs_relative_fault_tolerance_AND_initial_vs_updated_probabilities}, the a-priori ($p_{\mD,prio}()$) and the a-posteriori ($p_{\mD}()$) diagnoses probabilities might not only differ in terms of the probability values assigned to different diagnoses, but also in terms of the probability order of diagnoses. 
%
Incorporation of updated probabilities \emph{directly} into the hitting set tree algorithms to be used for the determination of leading diagnoses in the order prescribed by an updated probability measure is only possible if there is an additional update operator (besides Bayes' Theorem for adapting \emph{diagnoses} probabilities) that can be applied to \emph{formula} probabilities. For, the latter are exploited in the hitting set tree to assign probability weights to paths that are \emph{not yet diagnoses} (cf.\ $p_{nodes}()$ specified by Definition~\ref{def:p_node()} and the discussion of Formula~\ref{eq:path_prob_calc}) in order to guide the search for minimal diagnoses in best-first order. Updated \emph{diagnosis} probabilities are not helpful at all for this purpose. Devising a reasonable mechanism of updating formula probabilities seems to be hard mostly due to the lack of suitable data that might be collected during the debugging session to accomplish that. What would be imaginable during the debugging session is to try to learn something about the fault probability of \emph{syntactical elements} by examining the positive (all formulas are \emph{definitely} correct) and singleton negative (the single formula is \emph{definitely} incorrect) test cases. However, a drawback of such a strategy comes into effect when only syntactically very simple queries are used which is, for instance, the case in Example~\ref{example:query_computation} (see the definition of the \textsc{getEntailments} function there). From such queries not many useful insights concerning faulty syntactical elements might be gained. On the other hand, such queries are absolutely desirable from the point of view of how well a user might comprehend the formulas asked by the system. Hence, these two aspects seem to contradict each other. Still, it is a topic for future research to attempt to elaborate a solution for that issue.

\noindent\textbf{Facilitation of More Informative User Answers.} The debugging system described in this work is designed to get along with just a ``minimal'' feedback of a user regarding an asked query. That is, we assume the user' answer to a query $Q$ to be merely $\true$, i.e.\ each formula in $Q$ (or the conjunction of formulas in $Q$) must be entailed by the correct KB, or $\false$, i.e.\ at least one formula in $Q$ (or the conjunction of formulas in $Q$) must not be entailed by the correct KB. However, imagine a user being presented $Q$ and think of how they might proceed in order to come up with an answer to $Q$. The first observation is that, in order to respond by $\true$, a user must definitely scrutinize each single formula in $Q$ because otherwise they could never decide for sure whether the conjunction of all formulas in $Q$ is correct. Another observation is that a user might cease to go through the rest of the formulas in case they have already identified one that must not be an entailment of the desired KB. For, in this situation, the overall query $Q$ is already $\false$. This however indicates that at least one formula must be known to be correct or false whatever answer is given to $Q$. Therefore, we can usually expect a user to be able to give exactly this information, namely one formula in $Q$ that must be incorrect, additionally to answering by $\false$. This extra piece of information can be exploited to achieve better space and time efficiency in the context of diagnosis computation since knowing \emph{which} formula must definitely not be entailed gives more information that just a set of formulas of which we know that at least one among those is not entailed. 
%
Apart from that, there might be other pieces of additional information a user might be \emph{easily} able to give additionally to the ``minimal'' feedback we assume in this work. Proposing more efficient algorithms that exploit such tapes of additional information is on our future work agenda.
	 
\noindent\textbf{Usage of ``Positive-Impact'' Queries in Combination with \textsc{dynamicHS}.}	
	As we discussed in Section~\ref{sec:OverviewAndIntuition} in the context of Algorithm~\ref{algo:inter_onto_debug} in dynamic mode, an added test case might give rise to some pruning steps as well as it might induce the construction of new subtrees (where ``new'' means that these would be no subtress of a hitting set tree w.r.t.\ the DPI not including this test case). The latter situation occurs when ``completely new'' minimal conflict sets (those that are in no set-relationship with existing ones) are introduced by the addition of a test case. If this is the only impact of a test case, then this test case has only a negative influence on the time and space complexity of Algorithm~\ref{algo:inter_onto_debug} using \textsc{dynamicHS}. In other words, none of the invalidated minimal diagnoses (and no other nodes in the tree) are redundant; but all of them must additionally hit the set of ``completely new'' minimal conflict sets (in order to become diagnoses w.r.t.\ new DPI). Hence, in this case, the transition from one DPI to another including this test case results only in monotonic growth of the tree. If possible, such ``negative-impact test cases'' must be avoided. On the other hand, one must strive for the usage of ``positive-impact test cases'', i.e.\ those that only trigger tree pruning, but no tree expansion.  
Defining and studying properties that constitute such ``positive-impact test cases'' and ``negative-impact test cases'', respectively, and developing specialized algorithms for extracting exactly those types of queries that enable as substantial and effective pruning as possible in the context of \textsc{dynamicHS} is part of our already ongoing research. Note that a rough intuition of which properties make out a ``positive-impact test case'' is illustrated on the basis of an example in Section~\ref{sec:OverviewAndIntuition}.

\noindent\textbf{Finding the Right Expert to Answer a Query in a Collaborative KB Development Setting.}	As we mentioned in Chapter~\ref{chap:intro}, there are collaborative KB development projects such as the OBO Project\footnote{http://obo.sourceforge.net} and the NCI Thesaurus\footnote{http://nciterms.nci.nih.gov/ncitbrowser}, where many different people contribute to the specification of their knowledge in large KBs. In such a setting, it may be hard to decide who is the person that has the highest chance of being able to answer a concrete query correctly. The idea in such a scenario could be to use a combination of different measures such as educational level (e.g.\ professor versus PhD student) or hierarchy of contributors (e.g.\ senior user versus regular user), statistical information about past faults of a contributor (e.g., how many of the formulas originally authored by a person have been corrected by other persons of higher educational level) or provenance information regarding terms occurring in the query (who has authored most of the formulas where these terms occur) in order to learn an ``expert model'' and use it to devise some kind of recommender system \cite{jannach2010} that suggests which person to ask a particular query. 

Once established, such an expert model together with provenance information of KB formulas and other types of information discussed in Section~\ref{sec:prob_space_construction} could also be exploited when it comes to the definition of the fault information provided as input to our debugging system. An example of a system which enables the remote collaborative development of KBs (ontologies) and also provides logs of interesting usage data such a formula change logs and provenance information is Web Prot\'{e}g\'{e}~\cite{Tudorache2013}. 

\noindent\textbf{Methods for Query Selection without Computation of Diagnoses.} We are also working on ``conflict-based debugging'' methods that do not rely on the computation of leading diagnoses for query generation. Instead, queries might be generated directly from (minimal) conflict sets. Such methods might be used together with a boolean hitting set search tree (which was originally proposed by \cite{jiang2002} and optimized by \cite{Pill2012}) where the tree is regularly pruned using test cases such that tree branching is mostly or completely suppressed. In this manner, the tree remains small in size and all in all computes only a single diagnosis, i.e.\ the one consistent with all answered queries. Such an approach could be very space saving. Nevertheless, it is unclear whether the number of required queries and/or the computation time might increase. Implementing such an approach and answering these open questions is a topic on our future work agenda.  

\noindent\textbf{Employing Advanced Reasoning Techniques to Increase Debugging Efficiency.} To cope with application contexts where reasoning is the main obstacle for efficient debugging, a plan for future work is to integrate advances reasoning techniques into our system. 

For example, a modular combination of reasoners \cite{Romero2012} might be adopted. In such a system there are two sound reasoners are combined where one (R1, e.g.\ HermiT \cite{Shearer2008}) is complete for the full logic $\mathcal{L}$ (e.g.\ OWL~2 \cite{Grau2008a}) and the other one (R2, e.g.\ ELK \cite{kazakov2014}) is complete for only a fragment $\mathcal{L}' \subset \mathcal{L}$ (e.g.\ the OWL~2~EL profile \cite{Grau2008a}), but $\mathcal{L}'$ can be handles much more efficiently by R2. The system in \cite{Romero2012} could be used to assign the bulk of the workload on R2 while relying on R1 only if necessary. 

Another interesting approach might be to employ techniques introduced in \cite{Goncalves2012} for detecting so-called ``hot spots'' in KBs which, when deleted from the KB, lead to much more efficient reasoning. Since reasoning in our approaches is mostly applied to fractions of the faulty KB, we could possibly benefit from such an approach. For instance, queries are entailments of a set of different non-faulty fractions $\mo^*_i = (\mo \setminus \md_i) \cup \mb \cup U_{\Tp}$ of the original KB. Now, given that a hot spot $H$ is included, say in $\mb \cup U_{\Tp}$, then we might well delete $H$ from this subset of $\mo^*_i$ and might still obtain meaningful queries. The reason is that $H$ does not include any formulas in $U_{\mD}$ (where $\mD$ is the set of leading diagnoses) which are essential for query computation from the diagnosis discrimination point of view. Formulas in $\mb \cup U_{\Tp}$, on the other hand, are included in all non-faulty fractions $\mo^*_i$ and thus do not directly serve the discrimination between diagnoses. Since $U_{\mD}$ might be much smaller in size than $\mb \cup U_{\Tp}$ in many scenarios (due to a usually small number of leading diagnoses in $\mD$), there might be a high chance for hot spots to be located in $\mb \cup U_{\Tp}$ rather than in $U_{\mD}$.



==> eval.tex <==
\section{Evaluation} \label{sec:eval}
\textbf{Goals.}
This evaluation should demonstrate that (1) there is a significant discrepancy between existing strategies SPL and ENT concerning user effort where the winner depends on the quality of meta information, (2) RIO
exhibits superior average behavior compared to ENT and SPL w.r.t. the amount of user interaction required, irrespective of the quality of specified fault information, (3) RIO scales well and (4) its reaction time is well suited for an interactive debugging approach.

\noindent\textbf{Provenance of test data.} 
As data source for the evaluation we used faulty real-world ontologies produced by automatic ontology matching systems (cf.\ Example in Section~\ref{sec:basics}). 
%Ontology Matching is defined as:
Matching of two ontologies $\mo_i$ and $\mo_j$ is understood as detection of correspondences between elements of these ontologies~\cite{Shvaiko2012}: 
%
\begin{definition}[Ontology matching]\label{def:align}%~\cite{Shvaiko2012}
%Let $Q(\mo_i)\subseteq \Sig(\mo_i)$ and $Q(\mo_j)\subseteq \Sig(\mo_j)$ 
Let $Q(\mo)\subseteq \Sig(\mo)$ denote the set of matchable elements in an ontology $\mo$, where $\Sig(\mo)$ denotes the signature of $\mo$. An ontology matching operation determines an \emph{alignment} $\Al_{ij}$, which is a set of correspondences between matched ontologies $\mo_i$ and $\mo_j$. Each \emph{correspondence} is a 4-tuple $\tuple{x_i,x_j,r,v}$, such that $x_i \in Q(\mo_i)$, $x_j \in Q(\mo_j)$, $r$ is a semantic relation and $v \in [0,1]$ is a confidence value. We call $\mo_{i\Al j} := \mo_i \cup \N(\Al_{ij}) \cup \mo_j$ the \emph{aligned ontology} for $\mo_i$ and $\mo_j$ where $\N$ maps each correspondence to an axiom.
\end{definition}
%
Let in the following $Q(\mo)$ be the restriction to atomic concepts and roles in $\Sig(\mo)$, $r \in \setof{\sqsubseteq, \sqsupseteq, \equiv}$ and $\N$ the natural alignment semantics~\cite{MeilickeStuck2009} that maps correspondences one-to-one to axioms of the form $x_i~r~x_j$.
%
We evaluate RIO using aligned ontologies by the following reasons: (1) Matching results often cause inconsistency/incoherence of ontologies. (2) The (fault) structure of different ontologies obtained through matching generally varies due to different authors and matching systems involved in the genesis of these ontologies. (3) For the same reasons, it is hard to estimate the quality of fault probabilities, i.e. it is unclear which of the existing query selection strategies to chose for best performance. (4) Available reference mappings can be used as correct solutions of the debugging procedure.

\noindent\textbf{Test datasets.} We used two datasets D1 and D2: Each faulty aligned ontology $\mo_{i\Al j}$ in D1 is the result of applying one of four ontology matching systems to a set of six independently created ontologies in the domain of conference organization. For a given pair of ontologies $\mo_i\neq\mo_j$, each system produced an alignment $\Al_{ij}$. The average size of $\mo_{i\Al j}$ per matching system was between $312$ and $377$ axioms. D1 is a superset of the dataset used in \cite{Stuckenschmidt2008} for which all debugging systems under evaluation manifested correctness or scalability problems. D2, used to assess the scalability of RIO, is the set of ontologies
%\footnote{The raw data representing the output of matching systems was downloaded from http://bit.ly/Koh1NB. The reference alignment as well as the source ontologies Mouse and Human were downloaded from http://bit.ly/MU5Ca9.} 
from the ANATOMY track in the Ontology Alignment Evaluation Initiative\footnote{\texttt{http://oaei.ontologymatching.org}} (OAEI) 2011.5 \cite{Shvaiko2012}, which comprises two input ontologies $\mo_1$ (11545 axioms) and $\mo_2$ (4838 axioms). The size of the aligned ontologies generated by results of seven different matching systems was between 17530 and 17844 axioms.
\footnote{Source ontologies, produced alignments by each matcher, and reference alignments were downloaded from \texttt{http://bit.ly/Zffkow} (D1) and \texttt{http://bit.ly/Koh1NB} as well as \texttt{http://bit.ly/MU5Ca9} (D2).}
%Thus, D2 served to assess the scalability of RIO. 
%Note that the aligned ontologies output by five matching systems, i.e. CODI, CSA, MaasMtch, MapEVO and Aroma, could not be analyzed in the experiments. This was due to a coherent output produced by CODI and the problem that the reasoner was not able to find a model within acceptable time (2 hours) in the case of CSA, MaasMtch, MapEVO and Aroma. Similar reasoning problems were also reported in \cite{Ferrara2011}.

\noindent\textbf{Reference solutions.} For the dataset D1, based on a manually produced reference alignment $\mathcal{R}_{ij} \subseteq \Al_{ij}$ for ontologies $\mo_i,\mo_j$ (cf. \cite{Meilicke2008a}), we were able to fix a target diagnosis $\dt:=\N(\Al_{ij}\setminus\mathcal{R}_{ij})$ for each incoherent $\mo_{i\Al j}$. In cases where 
%$\mathcal{R}_{ij}$ 
$\dt$
represented a non-minimal diagnosis, 
it was randomly redefined 
as 
%the 
a
minimal diagnosis
%which was a subset of 
$\dt \subset \N(\Al_{ij}\setminus \mathcal{R}_{ij})$.
%we defined $\dt$ as the minimum cardinality diagnosis which was a subset of $\Al_{ij}\setminus \mathcal{R}_{ij}$. 
%
In case of D2, given the ontologies $\mo_1$ and $\mo_2$, the output $\Al_{12}$ of a matching system, and the correct reference alignment $\mathcal{R}_{12}$, we fixed $\dt$ as follows: We carried out (prior to the actual experiment) a debugging session with DPI $\tuple{\N(\Al_{12}\setminus \mathcal{R}_{12}),
        \mo_1\cup\mo_2\cup \N(\Al_{12} \cap \mathcal{R}_{12}),
        \emptyset,
        \emptyset}_{\setof{\text{coherence}}}$
and randomly chose one of the identified diagnoses as $\dt$.
%. From the set of identified diagnoses, we randomly defined one as $\dt$.
%Both ontologies $\mo_1$ and $\mo_2$ as well as the correctly extracted alignments $\Al_{12} \cap \mathcal{R}_{12}$ were placed in the background knowledge $\mb$. The incorrect correspondences $\Al_{12}\setminus \mathcal{R}_{12}$ were analyzed by the debugger. In this way, we identified a set of diagnoses, where each diagnosis is a subset of $\Al_{12}\setminus \mathcal{R}_{12}$. From this set of diagnoses, we randomly selected one diagnosis as $\dt$.

%\begin{figure*}[ht]
%\centering
%\subfigure[]{
%    %\vspace{-25mm}
%    %\tiny
%    {\fontsize{7pt}{8pt}\selectfont
%    \begin{tabular}{@{\extracolsep{-4pt}} l|c|c||c|c}
%																												& EXP-1		& EXP-2 	& EXP-3			& EXP-4			\\	\hline
%			$q_\text{SPL} < q_\text{ENT}$ 										& 11\%	  & 37\% 		& 	0\%			&   29\%		\\
%			$q_\text{ENT} < q_\text{SPL}$ 										& 81\%    &	56\% 	  & 	100\%		&		71\%		\\
%			$q_\text{SPL} = q_\text{ENT}$											& 7\%     &	7\% 	  & 	0\%			&		0\%			\\
%			$q_\text{RIO} < \min$															& 4\%	  	& 26\% 	  & 	29\%		&		71\%		\\
%			$q_\text{RIO} \leq \min$															& 74\%		& 74\% 	  & 	100\%		&		100\%		\\	\hline 
%				%\multicolumn{5}{c}{}	
%				%\\
%																											
%		\end{tabular}
%		}
%		\label{tab:best_strategies}
%}
%%\subfigure[]{
%%    %\rule{4cm}{3cm}
%%    \includegraphics[width=0.30\textwidth, trim=2mm 0mm 0mm 15mm]{diff_SPL_ENT_6.pdf}
%%    \label{fig:diff_SPL_ENT}
%%}
%\subfigure[]{
%%\tiny
%{\fontsize{7pt}{8pt}\selectfont
%\begin{tabular}{@{\extracolsep{-3pt}} l|c|c|c||c|c|c||c|c|c||c|c|c}
%		&  \multicolumn{3}{c||}{EXP-1}								  &  \multicolumn{3}{c||}{EXP-2}										&  \multicolumn{3}{c||}{EXP-3}					&  \multicolumn{3}{c}{EXP-4} & 
%		\hline
% 		& \textit{debug}					& \textit{react} 			& $q$ 					& 	\textit{debug} 				& \textit{react} 			& $q$ 					& \textit{debug} 				& \textit{react} 				& $q$ 					&  \textit{debug}				&  	\textit{react}				& $q$	\\\hline
%ENT &  1860					& 262 				& 3.67 					&  	1423					& 204 				& 5.26					& \textbf{60928}& 12367					& 5.86 					& 74463 				& 5629 					& 11.86	\\
%SPL &  \textbf{1427}& \textbf{159}& 5.70 					&  	\textbf{1237}	& \textbf{148}& 5.44					& 104910				&	\textbf{4786}	& 19.43 				& 98647 				& \textbf{4781}	& 18.29	\\
%RIO &  1592					& 286 				& \textbf{3.00}	&  	1749					&	245  				& \textbf{4.37}	& 62289					&	12825					& \textbf{5.43}	& \textbf{66895}& 8327 					& \textbf{8.14}	\\ \hline
%\end{tabular}
%}
%\label{tab:debug_react}
%}
%\vspace{-15pt}
%\caption[]{{
%%\fontsize{8pt}{7pt}\selectfont
%\footnotesize
%\textbf{\subref{tab:best_strategies}} Percentage rates indicating which strategy performed best/better w.r.t. the required user interaction, i.e. number of queries. EXP-1 and EXP-2 involved 27, EXP-3 and EXP-4 seven debugging sessions each. $q_{str}$ denotes the number of queries needed by strategy $str$ and $\min$ is an abbreviation for $\min(q_\text{SPL},q_\text{ENT})$. #
%\textbf{\subref{tab:debug_react}}
%Average time (ms) for the entire debugging session (\textit{debug}), average time (ms) between two successive queries (\textit{react}), and average number of queries ($q$) required by each strategy.}}
%\label{fig:best_diff}
%\end{figure*}
%
%\begin{figure*}[ht]
%\centering
%\subfigure[]{
%    %\vspace{-10pt}
%    \includegraphics[width=0.33\textwidth,trim=7mm -12mm 1mm 20mm]{query_conference_2.pdf}
%		\label{fig:query_conference}
%}
%\subfigure[]{
%    %\rule{4cm}{3cm}
%    \includegraphics[width=0.33\textwidth,trim=5mm 7mm 1mm 13mm]{query_anatomy_1.pdf}
%    \label{fig:query_anatomy}
%}
%\subfigure[]{
%    %\rule{4cm}{3cm}
%    \includegraphics[width=0.30\textwidth, trim=2mm -11mm 0mm 15mm]{diff_SPL_ENT_6.pdf}
%    \label{fig:diff_SPL_ENT}
%}
%\vspace{-17pt}
%\caption[]{{
%%\fontsize{8pt}{9pt}\selectfont 
%\footnotesize
%\textbf{\subref{fig:query_conference},\subref{fig:query_anatomy}} The bars show the avg. number of queries ($q$) needed by RIO, grouped by matching tools. The distance from the bar to the lower (upper) end of the whisker indicates the avg. difference of RIO to the queries needed by the per-session better (worse) strategy of SPL and ENT, respectively. \textbf{\subref{fig:diff_SPL_ENT}} Box-Whisker Plots presenting the distribution of overhead $(q_w-q_b)/q_b*100$ (in \%) per debugging session of the worse strategy $q_w := \max(q_\text{SPL},q_\text{ENT})$ compared to the better strategy $q_b := \min(q_\text{SPL},q_\text{ENT})$. Mean values are depicted by a cross.}}
%\label{fig:queries}
%\vspace{-10pt}
%\end{figure*}

\noindent\textbf{Test settings.} We conducted 4 experiments EXP-$i$ ($i=1,\dots,4$), the first two with dataset D1 and the other two with D2. In experiments 1 and 3 we simulated good fault probabilities by setting $p(\tax_k) := 0.001$ for $\tax_k \in \mo_i \cup \mo_j$ and $p(\tax_m):= 1-v_m$ for $\tax_m \in \Al_{ij}$, where $v_m$ is the confidence of the correspondence underlying $\tax_m$. Unreasonable fault information was used in experiments 2 and 4. In EXP-4 the following probabilities were defined: $p(\tax_k) := 0.01$ for $\tax_k \in \mo_i \cup \mo_j$ and $p(\tax_m):= 0.001$ for $\tax_m \in \Al_{ij}$. In EXP-2, in contrast, we used probability settings of EXP-1, but altered the target diagnosis $\dt$ in that we precomputed (before the actual experiment started) the 30 most probable minimal diagnoses, and from these we selected the diagnosis with the highest number of axioms $\tax_k \in \mo_{i\Al j} \setminus \N(\Al_{ij})$ as $\dt$. 

Throughout all four experiments, we set $|\mD|:=9$ (which proved to be a good trade-off between computation effort and representativeness of the leading diagnoses), $\sigma:=85\%$ and as input parameters for RIO we set $\uc:= 0.25$ and $[\underline{c},\overline{c}] := [\uc_{\min},\uc_{\max}] = [0,\frac{4}{9}]$. To let tests constitute the highest challenge for the evaluated methods, the initial DPI was specified as $\tuple{\mo_{i \Al j},\emptyset,\emptyset,\emptyset}_{\setof{\text{coherence}}}$, i.e. the entire search space was explored without adding parts of $\mo_{i \Al j}$ to 
%the background knowledge
$\mb$, although 
%the target diagnosis 
$\dt$ was always a subset of the alignment $\Al_{ij}$ only. In practice, given such prior knowledge, the search space could be severely restricted and debugging greatly accelerated.
% 
All tests were executed on a Core-i7 (3930K) 3.2Ghz, 32GB RAM with Ubuntu Server 11.04 and Java 6 installed. 
%installed.
\footnote{See \texttt{http://code.google.com/p/rmbd/wiki} for code and details.} 
%The number $|\mD|$ of leading diagnoses was set to 9 and $\sigma:=85\%$. As input parameters for RIO we set $\uc:= 0.25$ and $[\underline{c},\overline{c}] := [\uc_{\min},\uc_{\max}] = [0,\frac{4}{9}]$. For the tests we considered the most general setting, i.e. $\dt \subset \mo_{i \Al j}$. 

\noindent\textbf{Metrics.} Each experiment involved a debugging session of ENT, SPL as well as RIO for each ontology in the respective dataset. In each debugging run we measured the number of required queries ($q$) until $\dt$ was identified, the overall debugging time (\textit{debug}) assuming that queries are answered instantaneously and the reaction time (\textit{react}), i.e. the average time between two successive queries. The queries generated in the tests were answered by an automatic oracle by means of the target ontology $\mo_{i\Al j}\setminus \dt$.

\noindent\textbf{Observations.} 
The difference w.r.t. the number of queries per test run between the better and the worse strategy in \{SPL,ENT\} was absolutely significant, with a maximum of 2300\% in EXP-4 and averages of 190\% to 1145\% throughout all four experiments
(Figure~\ref{fig:diff_SPL_ENT}). 
Moreover, results show that varying quality of fault probabilities in \{\text{EXP-1},\text{EXP-3}\} compared to \{\text{EXP-2},\text{EXP-4}\} clearly affected the performance of ENT and SPL (see first two rows in 
Figure~\ref{tab:best_strategies}). This perfectly motivates the application of RIO.

Results of both experimental sessions, $\langle\text{EXP-1,EXP-2}\rangle$ and $\langle\text{EXP-3,EXP-4}\rangle$, are summarized in Figures~\ref{fig:query_conference} and \ref{fig:query_anatomy}, respectively. 
The figures show the (average) number of queries asked by RIO and the (average) differences to the number of queries needed by the per-session better and worse strategy in \{SPL,ENT\}, respectively. 
The results illustrate clearly that the average performance achieved by RIO was always substantially closer to the better than to the worse strategy. In both EXP-1 and EXP-2, throughout 74\% of 27 debugging sessions, RIO worked as efficiently as the best strategy (Figure \ref{tab:best_strategies}).  
In 26\% of the cases in EXP-2, RIO even outperformed both other strategies; in these cases, RIO could save more than 20\% of user interaction on average compared to the best other strategy. In one scenario in EXP-1, it took ENT 31 and SPL 13 queries to finish, whereas RIO required only 6 queries, which amounts to an improvement of more than 80\% and 53\%, respectively. In $\langle\text{EXP-3,EXP-4}\rangle$, the savings achieved by RIO were even more substantial. RIO manifested superior behavior to both other strategies in 29\% and 71\% of cases, respectively. Not less remarkable, in 100\% of the tests in EXP-3 and EXP-4, RIO was at least as efficient as the best other strategy. Recalling Figure~\ref{fig:diff_SPL_ENT}, this means that RIO can avoid query overheads of over 2000\%.
Table~\ref{tab:time_query}, which provides average values for $q$, \textit{react} and \textit{debug} per strategy,
demonstrates that RIO is the best choice in all experiments w.r.t. $q$. Consequently, RIO is suitable for both good 
and poor meta information.

As to time aspects, RIO manifested good performance, too. Since times consumed in $\langle\text{EXP-1,EXP-2}\rangle$ are almost negligible, consider the more meaningful results obtained in $\langle\text{EXP-3,EXP-4}\rangle$. While the best reaction time in both experiments was achieved by SPL, we can clearly see that SPL was significantly inferior to both ENT and RIO concerning $q$ and \textit{debug}. RIO revealed the best debugging time in EXP-4, and needed only $2.2\%$ more time than the best strategy (ENT) in EXP-3. However, if we assume the user being capable of reading and answering a query in, e.g., 30 sec on average, which is already quite fast, then the overall time savings of RIO compared to ENT in EXP-3 would already account for $5\%$. Doing the same thought experiment for EXP-4, RIO would save $25\%$ (w.r.t. ENT) and $50\%$ (w.r.t. SPL) of debugging time on average. All in all, the measured times confirm that RIO is well suited for \emph{interactive} debugging.


\begin{figure}[ht]
\centering
\subfigure[]{
    %\vspace{-25mm}
    \begin{tabular}[b]{@{\extracolsep{0pt}} l|c|c||c|c}
																												& EXP-1		& EXP-2 	& EXP-3			& EXP-4			\\	\hline
			$q_\text{SPL} < q_\text{ENT}$ 										& 11\%	  & 37\% 		& 	0\%			&   29\%		\\
			$q_\text{ENT} < q_\text{SPL}$ 										& 81\%    &	56\% 	  & 	100\%		&		71\%		\\
			$q_\text{SPL} = q_\text{ENT}$											& 7\%     &	7\% 	  & 	0\%			&		0\%			\\
			$q_\text{RIO} < \min$															& 4\%	  	& 26\% 	  & 	29\%		&		71\%		\\
			$q_\text{RIO} \leq \min$															& 74\%		& 74\% 	  & 	100\%		&		100\%		\\	\hline 
				\multicolumn{5}{c}{}	\\
																											
		\end{tabular}
		\vspace{15pt}
		\label{tab:best_strategies}
}
\subfigure[]{
    %\rule{4cm}{3cm}
    \includegraphics[width=0.45\textwidth, trim=2mm 0mm 0mm 15mm]{diff_SPL_ENT_6.pdf}
    \label{fig:diff_SPL_ENT}
}
\vspace{-8pt}
\caption[]{\textbf{\subref{tab:best_strategies}} Percentage rates indicating which strategy performed best/better w.r.t. the required user interaction, i.e. number of queries. EXP-1 and EXP-2 involved 27, EXP-3 and EXP-4 seven debugging sessions each. $q_{str}$ denotes the number of queries needed by strategy $str$ and $\min$ is an abbreviation for $\min(q_\text{SPL},q_\text{ENT})$. \textbf{\subref{fig:diff_SPL_ENT}} Box-Whisker Plots presenting the distribution of overhead $(q_w-q_b)/q_b*100$ (in \%) per debugging session of the worse strategy $q_w := \max(q_\text{SPL},q_\text{ENT})$ compared to the better strategy $q_b := \min(q_\text{SPL},q_\text{ENT})$. Mean values are depicted by a cross.}
\label{fig:best_diff}
\vspace{3pt}
%\hline
\end{figure}

\vspace{-2pt}

\begin{figure}[ht]
\centering
\subfigure[]{
    %\vspace{-15pt}
    \includegraphics[width=0.46\textwidth,trim=7mm -12mm 1mm 5mm]{query_conference_2.pdf}
		\label{fig:query_conference}
}
\subfigure[]{
    %\rule{4cm}{3cm}
    \includegraphics[width=0.46\textwidth,trim=5mm 7mm 1mm 10mm]{query_anatomy_1.pdf}
    \label{fig:query_anatomy}
}
\vspace{-9pt}
\caption[]{The bars show the avg. number of queries ($q$) needed by RIO, grouped by matching tools. The distance from the bar to the lower (upper) end of the whisker indicates the avg. difference of RIO to the queries needed by the per-session better (worse) strategy of SPL and ENT, respectively.}
\label{fig:queries}
\end{figure}



\vspace{-10pt}
\begin{table}
\centering
\begin{tabular}{@{\extracolsep{0pt}} l|c|c|c||c|c|c||c|c|c||c|c|c}
		&  \multicolumn{3}{c||}{EXP-1}								  &  \multicolumn{3}{c||}{EXP-2}										  														     &  \multicolumn{3}{c||}{EXP-3}					         &  \multicolumn{3}{c}{EXP-4} \\ 
		\hline
 		& \textit{debug}					& \textit{react} 			& $q$ 					& 	\textit{debug} 				& \textit{react} 			& $q$ 					& \textit{debug} 				& \textit{react} 				& $q$ 					&  \textit{debug}				&  	\textit{react}				& $q$	\\\hline
ENT &  1860					& 262 				& 3.67 					&  	1423					& 204 				& 5.26					& \textbf{60928}& 12367					& 5.86 					& 74463 				& 5629 					& 11.86	\\
SPL &  \textbf{1427}& \textbf{159}& 5.70 					&  	\textbf{1237}	& \textbf{148}& 5.44					& 104910				&	\textbf{4786}	& 19.43 				& 98647 				& \textbf{4781}	& 18.29	\\
RIO &  1592					& 286 				& \textbf{3.00}	&  	1749					&	245  				& \textbf{4.37}	& 62289					&	12825					& \textbf{5.43}	& \textbf{66895}& 8327 					& \textbf{8.14}	\\ \hline
\end{tabular}
\vspace{5pt}
\caption{Average time (ms) for the entire debugging session (\textit{debug}), average time (ms) between two successive queries (\textit{react}), and average number of queries ($q$) required by each strategy.} 
\vspace{-22pt}
\label{tab:time_query}
\end{table}



